LHAASO observation of Mrk 421 during 2021 March - 2024 March: a comprehensive VHE catalog of multi-timescale outbursts and its time average behavior

The Large High Altitude Air Shower Observatory (LHAASO) monitors sources within its field of view for up to 7 hours daily, achieving a duty cycle exceeding 98% and an annual point-source sensitivity of 1.5% Crab Units (CU) in the very high energy (VHE) band. This unbiased sky-survey mode facilitates systematic monitoring and investigation of outburst phenomena. In this paper, we present results from an unprecedented three-year monitoring campaign (March 2021--March 2024) of Mrk421 using LHAASO, spanning energies from 0.4 TeV to 20 TeV. We find that the blazar stayed in a quiescent state in 2021 and became active starting in 2022 with a total of 23 VHE outburst events identified, where the highest observed daily significance reaches $20\,\sigma$ with a flux equivalent to approximately 3.3~CU. LHAASO's continuous monitoring suggests the flaring occupancy of Mrk~421 to be around 14%. During long-term monitoring, multiwavelength (MWL) variability and correlation analyses are conducted using complementary data from Fermi-LAT, MAXI-GSC, Swift-XRT, and ZTF. A significant correlation ($>3\,\sigma$) is observed between X-ray and VHE bands with no detectable time lag, while the correlation between GeV and TeV bands is weaker. The flux distribution of the TeV emission during the quiescent state is different from that in the active state, implying the existence of two modes of energy dissipation in the blazar jet. Using simultaneous MWL data, we also analyzed both the long-term and outburst-period SEDs, and discussed the possible origin of the outburst events.

==> Science20240601.tex <==
Zhen Cao$^{1,2,3}$,
F. Aharonian$^{4,5}$,
Axikegu$^{6}$,
Y.X. Bai$^{1,3}$,
Y.W. Bao$^{7}$,
D. Bastieri$^{8}$,
X.J. Bi$^{1,2,3}$,
Y.J. Bi$^{1,3}$,
W. Bian$^{9}$,
A.V. Bukevich$^{10}$,
Q. Cao$^{11}$,
W.Y. Cao$^{12}$,
Zhe Cao$^{13,12}$,
J. Chang$^{14}$,
J.F. Chang$^{1,3,13}$,
A.M. Chen$^{9}$,
E.S. Chen$^{1,2,3}$,
H.X. Chen$^{15}$,
Liang Chen$^{16}$,
Lin Chen$^{6}$,
Long Chen$^{6}$,
M.J. Chen$^{1,3}$,
M.L. Chen$^{1,3,13}$,
Q.H. Chen$^{6}$,
S. Chen$^{17}$,
S.H. Chen$^{1,2,3}$,
S.Z. Chen$^{1,3}$,
T.L. Chen$^{18}$,
Y. Chen$^{7}$,
N. Cheng$^{1,3}$,
Y.D. Cheng$^{1,2,3}$,
M.C. Chu$^{19}$,
M.Y. Cui$^{14}$,
S.W. Cui$^{11}$,
X.H. Cui$^{20}$,
Y.D. Cui$^{21}$,
B.Z. Dai$^{17}$,
H.L. Dai$^{1,3,13}$,
Z.G. Dai$^{12}$,
Danzengluobu$^{18}$,
X.Q. Dong$^{1,2,3}$,
K.K. Duan$^{14}$,
J.H. Fan$^{8}$,
Y.Z. Fan$^{14}$,
J. Fang$^{17}$,
J.H. Fang$^{15}$,
K. Fang$^{1,3}$,
C.F. Feng$^{22}$,
H. Feng$^{1}$,
L. Feng$^{14}$,
S.H. Feng$^{1,3}$,
X.T. Feng$^{22}$,
Y. Feng$^{15}$,
Y.L. Feng$^{18}$,
S. Gabici$^{23}$,
B. Gao$^{1,3}$,
C.D. Gao$^{22}$,
Q. Gao$^{18}$,
W. Gao$^{1,3}$,
W.K. Gao$^{1,2,3}$,
M.M. Ge$^{17}$,
T.T. Ge$^{21}$,
L.S. Geng$^{1,3}$,
G. Giacinti$^{9}$,
G.H. Gong$^{24}$,
Q.B. Gou$^{1,3}$,
M.H. Gu$^{1,3,13}$,
F.L. Guo$^{16}$,
J. Guo$^{24}$,
X.L. Guo$^{6}$,
Y.Q. Guo$^{1,3}$,
Y.Y. Guo$^{14}$,
Y.A. Han$^{25}$,
O.A. Hannuksela$^{19}$,
M. Hasan$^{1,2,3}$,
H.H. He$^{1,2,3}$,
H.N. He$^{14}$,
J.Y. He$^{14}$,
Y. He$^{6}$,
Y.K. Hor$^{21}$,
B.W. Hou$^{1,2,3}$,
C. Hou$^{1,3}$,
X. Hou$^{26}$,
H.B. Hu$^{1,2,3}$,
Q. Hu$^{12,14}$,
S.C. Hu$^{1,3,27}$,
C. Huang$^{7}$,
D.H. Huang$^{6}$,
T.Q. Huang$^{1,3}$,
W.J. Huang$^{21}$,
X.T. Huang$^{22}$,
X.Y. Huang$^{14}$,
Y. Huang$^{1,2,3}$,
Y.Y. Huang$^{7}$,
X.L. Ji$^{1,3,13}$,
H.Y. Jia$^{6}$,
K. Jia$^{22}$,
H.B. Jiang$^{1,3}$,
K. Jiang$^{13,12}$,
X.W. Jiang$^{1,3}$,
Z.J. Jiang$^{17}$,
M. Jin$^{6}$,
M.M. Kang$^{28}$,
I. Karpikov$^{10}$,
D. Khangulyan$^{1,3}$,
D. Kuleshov$^{10}$,
K. Kurinov$^{10}$,
B.B. Li$^{11}$,
C.M. Li$^{7}$,
Cheng Li$^{13,12}$,
Cong Li$^{1,3}$,
D. Li$^{1,2,3}$,
F. Li$^{1,3,13}$,
H.B. Li$^{1,3}$,
H.C. Li$^{1,3}$,
Jian Li$^{12}$,
Jie Li$^{1,3,13}$,
K. Li$^{1,3}$,
S.D. Li$^{16,2}$,
W.L. Li$^{22}$,
W.L. Li$^{9}$,
X.R. Li$^{1,3}$,
Xin Li$^{13,12}$,
Y.Z. Li$^{1,2,3}$,
Zhe Li$^{1,3}$,
Zhuo Li$^{29}$,
E.W. Liang$^{30}$,
Y.F. Liang$^{30}$,
S.J. Lin$^{21}$,
B. Liu$^{12}$,
C. Liu$^{1,3}$,
D. Liu$^{22}$,
D.B. Liu$^{9}$,
H. Liu$^{6}$,
H.D. Liu$^{25}$,
J. Liu$^{1,3}$,
J.L. Liu$^{1,3}$,
M.Y. Liu$^{18}$,
R.Y. Liu$^{7}$,
S.M. Liu$^{6}$,
W. Liu$^{1,3}$,
Y. Liu$^{8}$,
Y.N. Liu$^{24}$,
Q. Luo$^{21}$,
Y. Luo$^{9}$,
H.K. Lv$^{1,3}$,
B.Q. Ma$^{29}$,
L.L. Ma$^{1,3}$,
X.H. Ma$^{1,3}$,
J.R. Mao$^{26}$,
Z. Min$^{1,3}$,
W. Mitthumsiri$^{31}$,
H.J. Mu$^{25}$,
Y.C. Nan$^{1,3}$,
A. Neronov$^{23}$,
K.C.Y. Ng$^{19}$,
L.J. Ou$^{8}$,
P. Pattarakijwanich$^{31}$,
Z.Y. Pei$^{8}$,
J.C. Qi$^{1,2,3}$,
M.Y. Qi$^{1,3}$,
B.Q. Qiao$^{1,3}$,
J.J. Qin$^{12}$,
A. Raza$^{1,2,3}$,
D. Ruffolo$^{31}$,
A. S\'aiz$^{31}$,
M. Saeed$^{1,2,3}$,
D. Semikoz$^{23}$,
L. Shao$^{11}$,
O. Shchegolev$^{10,32}$,
X.D. Sheng$^{1,3}$,
F.W. Shu$^{33}$,
H.C. Song$^{29}$,
Yu.V. Stenkin$^{10,32}$,
V. Stepanov$^{10}$,
Y. Su$^{14}$,
D.X. Sun$^{12,14}$,
Q.N. Sun$^{6}$,
X.N. Sun$^{30}$,
Z.B. Sun$^{34}$,
J. Takata$^{35}$,
P.H.T. Tam$^{21}$,
Q.W. Tang$^{33}$,
R. Tang$^{9}$,
Z.B. Tang$^{13,12}$,
W.W. Tian$^{2,20}$,
L.H. Wan$^{21}$,
C. Wang$^{34}$,
C.B. Wang$^{6}$,
G.W. Wang$^{12}$,
H.G. Wang$^{8}$,
H.H. Wang$^{21}$,
J.C. Wang$^{26}$,
Kai Wang$^{7}$,
Kai Wang$^{35}$,
L.P. Wang$^{1,2,3}$,
L.Y. Wang$^{1,3}$,
P.H. Wang$^{6}$,
R. Wang$^{22}$,
W. Wang$^{21}$,
X.G. Wang$^{30}$,
X.Y. Wang$^{7}$,
Y. Wang$^{6}$,
Y.D. Wang$^{1,3}$,
Y.J. Wang$^{1,3}$,
Z.H. Wang$^{28}$,
Z.X. Wang$^{17}$,
Zhen Wang$^{9}$,
Zheng Wang$^{1,3,13}$,
D.M. Wei$^{14}$,
J.J. Wei$^{14}$,
Y.J. Wei$^{1,2,3}$,
T. Wen$^{17}$,
C.Y. Wu$^{1,3}$,
H.R. Wu$^{1,3}$,
Q.W. Wu$^{35}$,
S. Wu$^{1,3}$,
X.F. Wu$^{14}$,
Y.S. Wu$^{12}$,
S.Q. Xi$^{1,3}$,
J. Xia$^{12,14}$,
G.M. Xiang$^{16,2}$,
D.X. Xiao$^{11}$,
G. Xiao$^{1,3}$,
Y.L. Xin$^{6}$,
Y. Xing$^{16}$,
D.R. Xiong$^{26}$,
Z. Xiong$^{1,2,3}$,
D.L. Xu$^{9}$,
R.F. Xu$^{1,2,3}$,
R.X. Xu$^{29}$,
W.L. Xu$^{28}$,
L. Xue$^{22}$,
D.H. Yan$^{17}$,
J.Z. Yan$^{14}$,
T. Yan$^{1,3}$,
C.W. Yang$^{28}$,
C.Y. Yang$^{26}$,
F. Yang$^{11}$,
F.F. Yang$^{1,3,13}$,
L.L. Yang$^{21}$,
M.J. Yang$^{1,3}$,
R.Z. Yang$^{12}$,
W.X. Yang$^{8}$,
Y.H. Yao$^{1,3}$,
Z.G. Yao$^{1,3}$,
L.Q. Yin$^{1,3}$,
N. Yin$^{22}$,
X.H. You$^{1,3}$,
Z.Y. You$^{1,3}$,
Y.H. Yu$^{12}$,
Q. Yuan$^{14}$,
H. Yue$^{1,2,3}$,
H.D. Zeng$^{14}$,
T.X. Zeng$^{1,3,13}$,
W. Zeng$^{17}$,
M. Zha$^{1,3}$,
B.B. Zhang$^{7}$,
F. Zhang$^{6}$,
H. Zhang$^{9}$,
H.M. Zhang$^{7}$,
H.Y. Zhang$^{17}$,
J.L. Zhang$^{20}$,
Li Zhang$^{17}$,
P.F. Zhang$^{17}$,
P.P. Zhang$^{12,14}$,
R. Zhang$^{14}$,
S.B. Zhang$^{2,20}$,
S.R. Zhang$^{11}$,
S.S. Zhang$^{1,3}$,
X. Zhang$^{7}$,
X.P. Zhang$^{1,3}$,
Y.F. Zhang$^{6}$,
Yi Zhang$^{1,14}$,
Yong Zhang$^{1,3}$,
B. Zhao$^{6}$,
J. Zhao$^{1,3}$,
L. Zhao$^{13,12}$,
L.Z. Zhao$^{11}$,
S.P. Zhao$^{14}$,
X.H. Zhao$^{26}$,
F. Zheng$^{34}$,
W.J. Zhong$^{7}$,
B. Zhou$^{1,3}$,
H. Zhou$^{9}$,
J.N. Zhou$^{16}$,
M. Zhou$^{33}$,
P. Zhou$^{7}$,
R. Zhou$^{28}$,
X.X. Zhou$^{1,2,3}$,
X.X. Zhou$^{6}$,
B.Y. Zhu$^{12,14}$,
C.G. Zhu$^{22}$,
F.R. Zhu$^{6}$,
H. Zhu$^{20}$,
K.J. Zhu$^{1,2,3,13}$,
Y.C. Zou$^{35}$,
X. Zuo$^{1,3}$,
(The LHAASO Collaboration)
$^{1}$ Key Laboratory of Particle Astrophysics \& Experimental Physics Division \& Computing Center, Institute of High Energy Physics, Chinese Academy of Sciences, 100049 Beijing, China\\
$^{2}$ University of Chinese Academy of Sciences, 100049 Beijing, China\\
$^{3}$ TIANFU Cosmic Ray Research Center, Chengdu, Sichuan,  China\\
$^{4}$ Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, 2 Dublin, Ireland \\
$^{5}$ Max-Planck-Institut for Nuclear Physics, P.O. Box 103980, 69029  Heidelberg, Germany\\
$^{6}$ School of Physical Science and Technology \&  School of Information Science and Technology, Southwest Jiaotong University, 610031 Chengdu, Sichuan, China\\
$^{7}$ School of Astronomy and Space Science, Nanjing University, 210023 Nanjing, Jiangsu, China\\
$^{8}$ Center for Astrophysics, Guangzhou University, 510006 Guangzhou, Guangdong, China\\
$^{9}$ Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China\\
$^{10}$ Institute for Nuclear Research of Russian Academy of Sciences, 117312 Moscow, Russia\\
$^{11}$ Hebei Normal University, 050024 Shijiazhuang, Hebei, China\\
$^{12}$ University of Science and Technology of China, 230026 Hefei, Anhui, China\\
$^{13}$ State Key Laboratory of Particle Detection and Electronics, China\\
$^{14}$ Key Laboratory of Dark Matter and Space Astronomy \& Key Laboratory of Radio Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China\\
$^{15}$ Research Center for Astronomical Computing, Zhejiang Laboratory, 311121 Hangzhou, Zhejiang, China\\
$^{16}$ Key Laboratory for Research in Galaxies and Cosmology, Shanghai Astronomical Observatory, Chinese Academy of Sciences, 200030 Shanghai, China\\
$^{17}$ School of Physics and Astronomy, Yunnan University, 650091 Kunming, Yunnan, China\\
$^{18}$ Key Laboratory of Cosmic Rays (Tibet University), Ministry of Education, 850000 Lhasa, Tibet, China\\
$^{19}$ Department of Physics, The Chinese University of Hong Kong, Shatin, New Territories, Hong Kong, China\\
$^{20}$ Key Laboratory of Radio Astronomy and Technology, National Astronomical Observatories, Chinese Academy of Sciences, 100101 Beijing, China\\
$^{21}$ School of Physics and Astronomy (Zhuhai) \& School of Physics (Guangzhou) \& Sino-French Institute of Nuclear Engineering and Technology (Zhuhai), Sun Yat-sen University, 519000 Zhuhai \& 510275 Guangzhou, Guangdong, China\\
$^{22}$ Institute of Frontier and Interdisciplinary Science, Shandong University, 266237 Qingdao, Shandong, China\\
$^{23}$ APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, CEA/IRFU, Observatoire de Paris, 119 75205 Paris, France\\
$^{24}$ Department of Engineering Physics \& Department of Astronomy, Tsinghua University, 100084 Beijing, China\\
$^{25}$ School of Physics and Microelectronics, Zhengzhou University, 450001 Zhengzhou, Henan, China\\
$^{26}$ Yunnan Observatories, Chinese Academy of Sciences, 650216 Kunming, Yunnan, China\\
$^{27}$ China Center of Advanced Science and Technology, Beijing 100190, China\\
$^{28}$ College of Physics, Sichuan University, 610065 Chengdu, Sichuan, China\\
$^{29}$ School of Physics, Peking University, 100871 Beijing, China\\
$^{30}$ Guangxi Key Laboratory for Relativistic Astrophysics, School of Physical Science and Technology, Guangxi University, 530004 Nanning, Guangxi, China\\
$^{31}$ Department of Physics, Faculty of Science, Mahidol University, Bangkok 10400, Thailand\\
$^{32}$ Moscow Institute of Physics and Technology, 141700 Moscow, Russia\\
$^{33}$ Center for Relativistic Astrophysics and High Energy Physics, School of Physics and Materials Science \& Institute of Space Science and Technology, Nanchang University, 330031 Nanchang, Jiangxi, China\\
$^{34}$ National Space Science Center, Chinese Academy of Sciences, 100190 Beijing, China\\
$^{35}$ School of Physics, Huazhong University of Science and Technology, Wuhan 430074, Hubei, China\\


==> affi.tex <==
\twocolumn

\vspace*{0.5cm}
\noindent $^{1}$ Key Laboratory of Particle Astrophysics \& Experimental Physics Division \& Computing Center, Institute of High Energy Physics, Chinese Academy of Sciences, 100049 Beijing, China\\
$^{2}$ University of Chinese Academy of Sciences, 100049 Beijing, China\\
$^{3}$ TIANFU Cosmic Ray Research Center, Chengdu, Sichuan,  China\\
$^{4}$ Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, 2 Dublin, Ireland \\
$^{5}$ Max-Planck-Institut for Nuclear Physics, P.O. Box 103980, 69029  Heidelberg, Germany\\
$^{6}$ School of Physical Science and Technology \&  School of Information Science and Technology, Southwest Jiaotong University, 610031 Chengdu, Sichuan, China\\
$^{7}$ School of Astronomy and Space Science, Nanjing University, 210023 Nanjing, Jiangsu, China\\
$^{8}$ Center for Astrophysics, Guangzhou University, 510006 Guangzhou, Guangdong, China\\
$^{9}$ Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China\\
$^{10}$ Institute for Nuclear Research of Russian Academy of Sciences, 117312 Moscow, Russia\\
$^{11}$ Hebei Normal University, 050024 Shijiazhuang, Hebei, China\\
$^{12}$ University of Science and Technology of China, 230026 Hefei, Anhui, China\\
$^{13}$ State Key Laboratory of Particle Detection and Electronics, China\\
$^{14}$ Key Laboratory of Dark Matter and Space Astronomy \& Key Laboratory of Radio Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China\\
$^{15}$ Research Center for Astronomical Computing, Zhejiang Laboratory, 311121 Hangzhou, Zhejiang, China\\
$^{16}$ Key Laboratory for Research in Galaxies and Cosmology, Shanghai Astronomical Observatory, Chinese Academy of Sciences, 200030 Shanghai, China\\
$^{17}$ School of Physics and Astronomy, Yunnan University, 650091 Kunming, Yunnan, China\\
$^{18}$ Key Laboratory of Cosmic Rays (Tibet University), Ministry of Education, 850000 Lhasa, Tibet, China\\
$^{19}$ Department of Physics, The Chinese University of Hong Kong, Shatin, New Territories, Hong Kong, China\\
$^{20}$ Key Laboratory of Radio Astronomy and Technology, National Astronomical Observatories, Chinese Academy of Sciences, 100101 Beijing, China\\
$^{21}$ School of Physics and Astronomy (Zhuhai) \& School of Physics (Guangzhou) \& Sino-French Institute of Nuclear Engineering and Technology (Zhuhai), Sun Yat-sen University, 519000 Zhuhai \& 510275 Guangzhou, Guangdong, China\\
$^{22}$ Institute of Frontier and Interdisciplinary Science, Shandong University, 266237 Qingdao, Shandong, China\\
$^{23}$ APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, CEA/IRFU, Observatoire de Paris, 119 75205 Paris, France\\
$^{24}$ Department of Engineering Physics \& Department of Astronomy, Tsinghua University, 100084 Beijing, China\\
$^{25}$ School of Physics and Microelectronics, Zhengzhou University, 450001 Zhengzhou, Henan, China\\
$^{26}$ Yunnan Observatories, Chinese Academy of Sciences, 650216 Kunming, Yunnan, China\\
$^{27}$ China Center of Advanced Science and Technology, Beijing 100190, China\\
$^{28}$ College of Physics, Sichuan University, 610065 Chengdu, Sichuan, China\\
$^{29}$ School of Physics, Peking University, 100871 Beijing, China\\
$^{30}$ Guangxi Key Laboratory for Relativistic Astrophysics, School of Physical Science and Technology, Guangxi University, 530004 Nanning, Guangxi, China\\
$^{31}$ Department of Physics, Faculty of Science, Mahidol University, Bangkok 10400, Thailand\\
$^{32}$ Moscow Institute of Physics and Technology, 141700 Moscow, Russia\\
$^{33}$ Center for Relativistic Astrophysics and High Energy Physics, School of Physics and Materials Science \& Institute of Space Science and Technology, Nanchang University, 330031 Nanchang, Jiangxi, China\\
$^{34}$ National Space Science Center, Chinese Academy of Sciences, 100190 Beijing, China\\
$^{35}$ School of Physics, Huazhong University of Science and Technology, Wuhan 430074, Hubei, China\\

==> name.tex <==
\author[LHAASO Collaboration]{\parbox{\textwidth}{
\normalsize
%name.tex
%\parbox{\textwidth}{
%\normalsize
Zhen Cao$^{1,2,3}$,
F. Aharonian$^{4,5}$,
Axikegu$^{6}$,
Y.X. Bai$^{1,3}$,
Y.W. Bao$^{7}$,
D. Bastieri$^{8}$,
X.J. Bi$^{1,2,3}$,
Y.J. Bi$^{1,3}$,
W. Bian$^{9}$,
A.V. Bukevich$^{10}$,
Q. Cao$^{11}$,
W.Y. Cao$^{12}$,
Zhe Cao$^{13,12}$,
J. Chang$^{14}$,
J.F. Chang$^{1,3,13}$,
A.M. Chen$^{9}$,
E.S. Chen$^{1,2,3}$,
H.X. Chen$^{15}$,
Liang Chen$^{16}$,
Lin Chen$^{6}$,
Long Chen$^{6}$,
M.J. Chen$^{1,3}$,
M.L. Chen$^{1,3,13}$,
Q.H. Chen$^{6}$,
S. Chen$^{17}$,
S.H. Chen$^{1,2,3}$,
S.Z. Chen$^{1,3}$,
T.L. Chen$^{18}$,
Y. Chen$^{7}$,
N. Cheng$^{1,3}$,
Y.D. Cheng$^{1,2,3}$,
M.C. Chu$^{19}$,
M.Y. Cui$^{14}$,
S.W. Cui$^{11}$,
X.H. Cui$^{20}$,
Y.D. Cui$^{21}$,
B.Z. Dai$^{17}$,
H.L. Dai$^{1,3,13}$,
Z.G. Dai$^{12}$,
Danzengluobu$^{18}$,
X.Q. Dong$^{1,2,3}$,
K.K. Duan$^{14}$,
J.H. Fan$^{8}$,
Y.Z. Fan$^{14}$,
J. Fang$^{17}$,
J.H. Fang$^{15}$,
K. Fang$^{1,3}$,
C.F. Feng$^{22}$\thanks{\href{mailto: fengcf@sdu.edu.cn}{fengcf@sdu.edu.cn}},
H. Feng$^{1}$,
L. Feng$^{14}$,
S.H. Feng$^{1,3}$,
X.T. Feng$^{22}$,
Y. Feng$^{15}$,
Y.L. Feng$^{18}$,
S. Gabici$^{23}$,
B. Gao$^{1,3}$,
C.D. Gao$^{22}$,
Q. Gao$^{18}$,
W. Gao$^{1,3}$,
W.K. Gao$^{1,2,3}$,
M.M. Ge$^{17}$,
T.T. Ge$^{21}$,
L.S. Geng$^{1,3}$,
G. Giacinti$^{9}$,
G.H. Gong$^{24}$,
Q.B. Gou$^{1,3}$,
M.H. Gu$^{1,3,13}$,
F.L. Guo$^{16}$,
J. Guo$^{24}$,
X.L. Guo$^{6}$,
Y.Q. Guo$^{1,3}$,
Y.Y. Guo$^{14}$,
Y.A. Han$^{25}$,
O.A. Hannuksela$^{19}$,
M. Hasan$^{1,2,3}$,
H.H. He$^{1,2,3}$,
H.N. He$^{14}$,
J.Y. He$^{14}$,
Y. He$^{6}$,
Y.K. Hor$^{21}$,
B.W. Hou$^{1,2,3}$,
C. Hou$^{1,3}$,
H.B. Hu$^{1,2,3}$,
Q. Hu$^{12,14}$,
S.C. Hu$^{1,3,27}$,
C. Huang$^{7}$,
D.H. Huang$^{6}$,
T.Q. Huang$^{1,3}$,
W.J. Huang$^{21}$,
X.T. Huang$^{22}$,
X.Y. Huang$^{14}$,
Y. Huang$^{1,2,3}$,
Y.Y. Huang$^{7}$,
X.L. Ji$^{1,3,13}$,
H.Y. Jia$^{6}$,
K. Jia$^{22}$,
H.B. Jiang$^{1,3}$,
K. Jiang$^{13,12}$,
X.W. Jiang$^{1,3}$,
Z.J. Jiang$^{17}$,
M. Jin$^{6}$,
M.M. Kang$^{28}$,
I. Karpikov$^{10}$,
D. Khangulyan$^{1,3}$,
D. Kuleshov$^{10}$,
K. Kurinov$^{10}$,
B.B. Li$^{11}$,
C.M. Li$^{7}$,
Cheng Li$^{13,12}$,
Cong Li$^{1,3}$,
D. Li$^{1,2,3}$,
F. Li$^{1,3,13}$,
H.B. Li$^{1,3}$,
H.C. Li$^{1,3}$,
Jian Li$^{12}$,
Jie Li$^{1,3,13}$,
K. Li$^{1,3}$,
S.D. Li$^{16,2}$,
W.L. Li$^{22}$,
W.L. Li$^{9}$,
X.R. Li$^{1,3}$,
Xin Li$^{13,12}$,
Y.Z. Li$^{1,2,3}$,
Zhe Li$^{1,3}$,
Zhuo Li$^{29}$,
E.W. Liang$^{30}$,
Y.F. Liang$^{30}$,
S.J. Lin$^{21}$,
B. Liu$^{12}$,
C. Liu$^{1,3}$,
D. Liu$^{22}$,
D.B. Liu$^{9}$,
H. Liu$^{6}$,
H.D. Liu$^{25}$,
J. Liu$^{1,3}$,
J.L. Liu$^{1,3}$,
M.Y. Liu$^{18}$,
R.Y. Liu$^{7}$,
S.M. Liu$^{6}$,
W. Liu$^{1,3}$,
Y. Liu$^{8}$,
Y.N. Liu$^{24}$,
Q. Luo$^{21}$,
Y. Luo$^{9}$,
H.K. Lv$^{1,3}$,
B.Q. Ma$^{29}$,
L.L. Ma$^{1,3}$,
X.H. Ma$^{1,3}$,
J.R. Mao$^{26}$\thanks{\href{mailto:jirongmao@mail.ynao.ac.cn}{jirongmao@mail.ynao.ac.cn}}，
Z. Min$^{1,3}$,
W. Mitthumsiri$^{31}$,
H.J. Mu$^{25}$,
Y.C. Nan$^{1,3}$,
A. Neronov$^{23}$,
K.C.Y. Ng$^{19}$,
L.J. Ou$^{8}$,
P. Pattarakijwanich$^{31}$,
Z.Y. Pei$^{8}$,
J.C. Qi$^{1,2,3}$,
M.Y. Qi$^{1,3}$,
B.Q. Qiao$^{1,3}$,
J.J. Qin$^{12}$,
A. Raza$^{1,2,3}$,
D. Ruffolo$^{31}$,
A. S\'aiz$^{31}$,
M. Saeed$^{1,2,3}$,
D. Semikoz$^{23}$,
L. Shao$^{11}$,
O. Shchegolev$^{10,32}$,
X.D. Sheng$^{1,3}$,
F.W. Shu$^{33}$,
H.C. Song$^{29}$,
Yu.V. Stenkin$^{10,32}$,
V. Stepanov$^{10}$,
Y. Su$^{14}$,
D.X. Sun$^{12,14}$,
Q.N. Sun$^{6}$,
X.N. Sun$^{30}$,
Z.B. Sun$^{34}$,
J. Takata$^{35}$,
P.H.T. Tam$^{21}$,
Q.W. Tang$^{33}$,
R. Tang$^{9}$,
Z.B. Tang$^{13,12}$,
W.W. Tian$^{2,20}$,
L.H. Wan$^{21}$,
C. Wang$^{34}$,
C.B. Wang$^{6}$,
G.W. Wang$^{12}$,
H.G. Wang$^{8}$,
H.H. Wang$^{21}$,
J.C. Wang$^{26}$,
Kai Wang$^{7}$,
Kai Wang$^{35}$,
L.P. Wang$^{1,2,3}$,
L.Y. Wang$^{1,3}$,
P.H. Wang$^{6}$,
R. Wang$^{22}$\thanks{\href{mailto:ranw@mail.sdu.edu.cn}{ranw@mail.sdu.edu.cn}},
W. Wang$^{21}$,
X.G. Wang$^{30}$,
X.Y. Wang$^{7}$,
Y. Wang$^{6}$,
Y.D. Wang$^{1,3}$,
Y.J. Wang$^{1,3}$,
Z.H. Wang$^{28}$,
Z.X. Wang$^{17}$,
Zhen Wang$^{9}$,
Zheng Wang$^{1,3,13}$,
D.M. Wei$^{14}$,
J.J. Wei$^{14}$,
Y.J. Wei$^{1,2,3}$,
T. Wen$^{17}$,
C.Y. Wu$^{1,3}$,
H.R. Wu$^{1,3}$,
Q.W. Wu$^{35}$,
S. Wu$^{1,3}$,
X.F. Wu$^{14}$,
Y.S. Wu$^{12}$,
S.Q. Xi$^{1,3}$,
J. Xia$^{12,14}$,
G.M. Xiang$^{16,2}$,
D.X. Xiao$^{11}$,
G. Xiao$^{1,3}$,
Y.L. Xin$^{6}$,
Y. Xing$^{16}$,
D.R. Xiong$^{26}$,
Z. Xiong$^{1,2,3}$,
D.L. Xu$^{9}$,
R.F. Xu$^{1,2,3}$,
R.X. Xu$^{29}$,
W.L. Xu$^{28}$,
L. Xue$^{22}$,
D.H. Yan$^{17}$,
J.Z. Yan$^{14}$,
T. Yan$^{1,3}$,
C.W. Yang$^{28}$,
C.Y. Yang$^{26}$\thanks{\href{mailto:chyyo@ynao.ac.cn}{chyy@ynao.ac.cn}},
F. Yang$^{11}$,
F.F. Yang$^{1,3,13}$,
L.L. Yang$^{21}$,
M.J. Yang$^{1,3}$,
R.Z. Yang$^{12}$,
W.X. Yang$^{8}$,
Y.H. Yao$^{1,3}$,
Z.G. Yao$^{1,3}$,
L.Q. Yin$^{1,3}$,
N. Yin$^{22}$,
X.H. You$^{1,3}$,
Z.Y. You$^{1,3}$,
Y.H. Yu$^{12}$,
Q. Yuan$^{14}$,
H. Yue$^{1,2,3}$,
H.D. Zeng$^{14}$,
T.X. Zeng$^{1,3,13}$,
W. Zeng$^{17}$,
M. Zha$^{1,3}$\thanks{\href{mailto:zham@ihep.ac.cn}{zham@ihep.ac.cn}},
B.B. Zhang$^{7}$,
F. Zhang$^{6}$,
H. Zhang$^{9}$,
H.M. Zhang$^{7}$,
H.Y. Zhang$^{17}$,
J.L. Zhang$^{20}$,
Li Zhang$^{17}$,
P.F. Zhang$^{17}$,
P.P. Zhang$^{12,14}$,
R. Zhang$^{14}$,
S.B. Zhang$^{2,20}$,
S.R. Zhang$^{11}$,
S.S. Zhang$^{1,3}$,
X. Zhang$^{7}$,
X.P. Zhang$^{1,3}$,
Y.F. Zhang$^{6}$,
Yi Zhang$^{1,14}$,
Yong Zhang$^{1,3}$,
B. Zhao$^{6}$,
J. Zhao$^{1,3}$,
L. Zhao$^{13,12}$,
L.Z. Zhao$^{11}$,
S.P. Zhao$^{14}$,
X.H. Zhao$^{26}$,
F. Zheng$^{34}$,
W.J. Zhong$^{7}$,
B. Zhou$^{1,3}$,
H. Zhou$^{9}$,
J.N. Zhou$^{16}$,
M. Zhou$^{33}$,
P. Zhou$^{7}$,
R. Zhou$^{28}$,
X.X. Zhou$^{1,2,3}$,
X.X. Zhou$^{6}$,
B.Y. Zhu$^{12,14}$,
C.G. Zhu$^{22}$,
F.R. Zhu$^{6}$,
H. Zhu$^{20}$,
K.J. Zhu$^{1,2,3,13}$,
Y.C. Zou$^{35}$,
X. Zuo$^{1,3}$,(LHAASO Collaboration)
}
%\newauthor (Affiliations can be found after the references)
}


